Homotopy Colimits of Algebras Over Cat-Operads and Iterated Loop Spaces

We extend Thomason's homotopy colimit construction in the category of permutative categories to categories of algebras over an arbitrary $\Cat$ operad and analyze its properties. We then use this homotopy colimit to prove that the classifying space functor induces an equivalence between the category of $n$-fold monoidal categories and the category of $\mathcal{C}_n$-spaces after formally inverting certain classes of weak equivalences, where $\mathcal{C}_n$ is the little $n$-cubes operad. As a consequence we obtain an equivalence of the categories of $n$-fold monoidal categories and the category of $n$-fold loop spaces and loop maps after localization with respect to some other class of weak equivalences. We recover Thomason's corresponding result about infinite loop spaces and obtain related results about braided monoidal categories and 2-fold loop spaces.

==> abstract.tex <==
Abstract:

We extend Thomason's homotopy colimit construction in the category
of permutative categories to categories of algebras over an arbitrary
$\Cat$ operad and analyze its properties. We then use this homotopy colimit to 
prove that the classifying space functor induces an equivalence
between the category of $n$-fold monoidal categories and the category
of $\cC_n$-spaces after formally inverting certain classes of weak equivalences,
where $\cC_n$ is the little $n$-cubes operad. As a consequence we obtain
an equivalence of the categories of $n$-fold monoidal categories and the
category of $n$-fold loop spaces and loop maps after localization with 
respect to some other class of weak equivalences. We recover
Thomason's corresponding result about infinite loop spaces and
obtain related results about braided monoidal categories and $2$-fold
loop spaces.


 




